An Implementation of Homotopy Type Theory in Isabelle/Pure

In this Masters thesis we present an implementation of a fragment of "book HoTT" as an object logic for the interactive proof assistant Isabelle. We also give a mathematical description of the underlying theory of the Isabelle/Pure logical framework, and discuss various issues and design decisions that arise when attempting to encode intensional dependent type theory with universes inside a simple type-theoretic logical foundation.

==> chapter5.tex <==
\chapter{}

\vspace{15cm}

Code, issues and documentation updated at \url{https://github.com/jaycech3n/Isabelle-HoTT}.

